A real-time, hardware agnostic framework for close-up branch reconstruction using RGB data

Creating accurate 3D models of tree topology is an important task for tree pruning. The 3D model is used to decide which branches to prune and then to execute the pruning cuts. Previous methods for creating 3D tree models have typically relied on point clouds, which are often computationally expensive to process and can suffer from data defects, especially with thin branches. In this paper, we propose a method for actively scanning along a primary tree branch, detecting secondary branches to be pruned, and reconstructing their 3D geometry using just an RGB camera mounted on a robot arm. We experimentally validate that our setup is able to produce primary branch models with 4-5 mm accuracy and secondary branch models with 15 degrees orientation accuracy with respect to the ground truth model. Our framework is real-time and can run up to 10 cm/s with no loss in model accuracy or ability to detect secondary branches.

==> results_old.tex <==
\begin{table*}[]
\centering
\begin{tabular}{|l|ccccc|cccc|}
\hline
 & \multicolumn{5}{|c|}{Simulated Experiments} & \multicolumn{4}{|c|}{Real Experiments} \\ \hline
Lookat Angle \degree         & 0                 & 22.5              & 45                & 22.5              & 45 & 22.5 & 0 & 0 & 0               \\
Rotation Freq              & 0                 & 1.5               & 1.5               & 2.5               & 2.5 & 1.5 & 0 & 0 & 0               \\
Speed & N/A & N/A & N/A & N/A & N/A & 0.05 & 0.02 & 0.05 & 0.10 \\
\hline
% Completed                  & 100\%             & 100\%             & 98.3\%            & 100\%             & 98.3\%            \\
PB Resid. (mm)       & 3.5 (4.0)         & 4.2 (4.9)      & 4.5 (8.9)      & 3.8 (3.7)      & 4.8 (7.5) & 4.3 (4.6) & 11.9 (15.9) & 6.5 (13.1) & 4.7 (7.5)     \\
PB Rad. Error \%     & 6 (10)        & 5 (9)    & 6 (9)    & 5 (7)    & 6 (9) & 18 (15) & 16 (31) & 16 (18) & 19 (18)   \\ \hline
SB $\angle$ Error \degree & 13 (8)       & 16 (11)      & 15 (9)       & 15 (10)       & 17 (10) & 13 (8) & 17 (13) & 11 (5) & 15 (6) \\
SB Detection \%          & 91            & 95            & 91            & 95            & 91 & 76 & 76 & 73 & 76           \\
SB Len Error \%            & 5 (91)   & 11 (84)  & -4 (32) & 4 (75)  & 4 (51) & N/A & N/A & N/A & N/A  \\
SB Rad. Error \%         & -13 (16) & -13 (15) & -12 (16) & -12 (15) & -11 (13) & N/A & N/A & N/A & N/A\\
     \hline
\end{tabular}
\caption{Results of the simulated and real experiments for each parameter set (PB = primary branch, SB = secondary branch, Resid = residual, Rad. = radius). Standard deviation values are given in parentheses.}
\label{table:results_combined}
\end{table*}


==> results_table_real.tex <==
\begin{table*}[]
\centering
\begin{tabular}{|l|c|ccc|}
\hline
Lookat Angle (deg)         & 22.5             & 0                & 0                & 0                \\
Rotation Freq              & 1.5              & 0                & 0                & 0                \\
Speed (m/s)                & 0.05             & 0.02             & 0.05             & 0.10             \\ \hline
Leader Residual (mm)       & 4.27 $\pm$ 4.58    & 11.90 $\pm$ 15.86   & 6.54 $\pm$ 13.14   & 4.65 $\pm$ 7.54    \\
Leader Radius Error \%     & 18.2\% $\pm$ 15.0\% & 16.4\% $\pm$ 30.8\% & 16.1\% $\pm$ 18.2\% & 18.8\% $\pm$ 18.1\% \\ \hline
SB Detection Rate          & 76\%                & 76\%                  & 73\%                  & 76\%                 \\
SB Orientation Error (deg) & 13.0 $\pm$ 7.6      & 16.5 $\pm$ 12.6     & 10.5 $\pm$ 4.9      & 14.8 $\pm$ 6.1     \\ \hline
\end{tabular}
\caption{Results of the real experiments for each parameter set. Standard deviation values are given to the right of the $\pm$ symbol.}
\label{table:results_real}
\end{table*}

==> results_table_sim.tex <==



% \begin{table*}[]
% \centering
% \begin{tabular}{|l|c|cc|cc|}
% \hline
% Lookat Angle (deg)         & 0                 & 22.5              & 45                & 22.5              & 45                \\
% Rotation Freq              & 0                 & 1.5               & 1.5               & 2.5               & 2.5               \\ \hline
% Completed                  & 100\%             & 100\%             & 98.3\%            & 100\%             & 98.3\%            \\
% Leader Residual (mm)       & 3.49 $\pm$ 3.95      & 4.21 $\pm$ 4.92      & 4.50 $\pm$ 8.93      & 3.82 $\pm$ 3.68      & 4.79 $\pm$ 7.48      \\
% Leader Radius Error \%     & 6.4\% $\pm$ 10.3\%   & 5.1\% $\pm$ 8.5\%    & 5.7\% $\pm$ 9.0\%    & 5.3\% $\pm$ 7.3\%    & 6.3\% $\pm$ 9.0\%    \\ \hline
% SB Detection Rate          & 90.7\%            & 95.3\%            & 90.5\%            & 94.7\%            & 91.3\%            \\
% SB Length Error            & 5.2\% $\pm$ 90.7\%   & 10.5\% $\pm$ 83.7\%  & -4.0\% $\pm$ 32.3\%  & 3.9\% $\pm$ 74.7\%   & 3.6\% $\pm$ 50.6\%   \\
% SB Radius Error \%         & -13.0\% $\pm$ 15.8\% & -13.1\% $\pm$ 15.4\% & -12.4\% $\pm$ 16.1\% & -11.7\% $\pm$ 15.0\% & -10.9\% $\pm$ 12.8\% \\
% SB Orientation Error (deg) & 13.1 $\pm$ 8.3       & 15.9 $\pm$ 10.8      & 15.3 $\pm$ 9.1       & 15.1 $\pm$ 9.8       & 16.6 $\pm$ 10.0 \\     \hline
% \end{tabular}
% \caption{Results of the simulated experiments for each parameter set. Standard deviation values are given to the right of the $\pm$ symbol.}
% \label{table:results_sim}
% \end{table*}

==> todo.tex <==
data analysis still to do
Sim - need to get out reconstructed 2d branches (pts plus radii) to calculate residual error for the secondary branches 

For lab data:
Same as above, but also need either to measure the real branches if at all possible and average those radii errors

For Orchard data
Same as above for radii (match point radii measures to which branch they came from)

Figures

Fig 6: Add orchard setup
insets boudnaries 
3 image lab expt


separate image

Figure 7 types of failures


replace 1
Table 1: Extend with orchard data

Text changes:
Change text on measures to be just 
1) Length error/non orthogonal -> do it in camera frame
2) redo residual

[Cindy] Text editing to bring length down


Table

Angle
Rotat
Freq
Dist

PB Resid
PB Rad

SB  Detection
SB Resid
SB Rad

Two more columns for orchard

box plot: for best one residual error
